Bag of Genres for Video Retrieval

Often, videos are composed of multiple concepts or even genres. For instance, news videos may contain sports, action, nature, etc. Therefore, encoding the distribution of such concepts/genres in a compact and effective representation is a challenging task. In this sense, we propose the Bag of Genres representation, which is based on a visual dictionary defined by a genre classifier. Each visual word corresponds to a region in the classification space. The Bag of Genres video vector contains a summary of the activations of each genre in the video content. We evaluate the proposed method for video genre retrieval using the dataset of MediaEval Tagging Task of 2012 and for video event retrieval using the EVVE dataset. Results show that the proposed method achieves results comparable or superior to state-of-the-art methods, with the advantage of providing a much more compact representation than existing features.

==> Makefile <==
### Makefile
### $Id: Makefile,v 1.11 2006/06/26 04:51:29 jurandy Exp $

CP = cp
MV = mv
RM = rm

EGREP = egrep

LATEX = latex
BIBTEX = bibtex
DVIPS = dvips
PS2PDF = ps2pdf
PDFLATEX = pdflatex

BIBFLAGS = -min-crossrefs=32768
DVIFLAGS = -t letter -Ppdf -Pbuiltin35 -G0
PSFLAGS = -sPAPERSIZE=letter -dCompatibilityLevel=1.2 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress
PDFFLAGS = -shell-escape


RERUN = "Rerun to get (cross-references|the bars) right"
RERUNBIB = "No file.*\.bbl"

SRC = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)

all: install clean

install: pdftex

uninstall:
	$(RM) -f $(SRC:%.tex=%.dvi) $(SRC:%.tex=%.ps) $(SRC:%.tex=%.pdf)

%.dvi:	%.tex
	$(LATEX) $<
	$(EGREP) -c $(RERUNBIB) $*.log && $(BIBTEX) $(BIBFLAGS) $* ; true
	while ( $(LATEX) $< ; $(EGREP) -c $(RERUN) $*.log ) do true ; done
	$(EGREP) -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:	%.dvi
	$(DVIPS) $(DVIFLAGS) $< -o $@

%.dpp:	%.ps
	$(PS2PDF)  $(PSFLAGS) $<

%.pdf:	%.tex
	$(PDFLATEX) $(PDFFLAGS) $<
	$(EGREP) -c $(RERUNBIB) $*.log && $(BIBTEX) $(BIBFLAGS) $* ; true
	while ( $(PDFLATEX) $(PDFFLAGS) $< ; $(EGREP) -c $(RERUN) $*.log ) do true ; done
	$(EGREP) -i "(Reference|Citation).*undefined" $*.log ; true

%.pic:	%.dpp
	$(MV) $*.pdf $*-pics.pdf

%.p4f:	%.pic %.pdf
	$(RM) -f $*.dvi $*.ps $*-pics.pdf

dvi:	$(SRC:%.tex=%.dvi)
ps:	$(SRC:%.tex=%.ps)
dvips:	$(SRC:%.tex=%.dpp)
pdftex:	$(SRC:%.tex=%.pdf)
ps4pdf:	$(SRC:%.tex=%.p4f)

clean:
	$(RM) -f *-pics.* core *.core *.log *.aux *.toc *.lo[fpta] \
	*.blg *.brf *.ind *.ilg *.idx *.glo *.gls *.nav *.snm *.pfg *.out

### Makefile ends here.


